Sound and Complete Bidirectional Typechecking for Higher-Rank Polymorphism with Existentials and Indexed Types

Bidirectional typechecking, in which terms either synthesize a type or are checked against a known type, has become popular for its applicability to a variety of type systems, its error reporting, and its ease of implementation. Following principles from proof theory, bidirectional typing can be applied to many type constructs. The principles underlying a bidirectional approach to indexed types (generalized algebraic datatypes) are less clear. Building on proof-theoretic treatments of equality, we give a declarative specification of typing based on focalization. This approach permits declarative rules for coverage of pattern matching, as well as support for first-class existential types using a focalized subtyping judgment. We use refinement types to avoid explicitly passing equality proofs in our term syntax, making our calculus similar to languages such as Haskell and OCaml. We also extend the declarative specification with an explicit rules for deducing when a type is principal, permitting us to give a complete declarative specification for a rich type system with significant type inference. We also give a set of algorithmic typing rules, and prove that it is sound and complete with respect to the declarative system. The proof requires a number of technical innovations, including proving soundness and completeness in a mutually recursive fashion.

==> extensions.tex <==
\section{Extensions}
\Label{sec:extensions}



%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%



%
%
%


==> fig-asymmetric-instantiation.tex <==
\begin{figure*}[htbp]
      \judgbox{\instjudgl{\Gamma}{\ahat}{A}{\Delta}}%
         {Under input context $\Gamma$,
           instantiate $\ahat$ such that $\ahat \subtype A$, 
           with output context $\Delta$}
      \begin{mathpar}
        \Infer{\InstLSolve}
                { \Gamma \entails \tau} %
                { \instjudgl{\Gamma, \ahat, \Gamma'}
                            {\ahat}
                            {\tau}
                            {\Gamma, \hypeq{\ahat}{\tau}, \Gamma'}
                 }
        \and
        \Infer{\InstLReach}
                { }
                {\instjudgl{\Gamma[\ahat][\bhat]}
                            {\ahat}
                            {\bhat}
                            {\Gamma[\ahat][\hypeq{\bhat}{\ahat}]}}
        \and
        \Infer{\InstLArr}
                {\instjudgr{\Gamma[\ahat_2, \ahat_1, \hypeq{\ahat}{\ahat_1 \arr \ahat_2}]}
                            {\ahat_1}
                            {A_1}
                            {\Theta} \\
                 \instjudgl{\Theta}
                            {\ahat_2}
                            {[\Theta]A_2}
                            {\Delta}}
                {\instjudgl{\Gamma[\ahat]}
                            {\ahat}
                            {A_1 \arr A_2}
                            {\Delta}}
        \and
        \Infer{\InstLAllR}
              {\instjudgl{\Gamma[\ahat], \beta:\sort}{\ahat}{B}{\Delta, \beta:\sort, \Delta'}}
              {\instjudgl{\Gamma[\ahat]}{\ahat}{\alltype{\beta:\sort}{B}}{\Delta}}
        \\
        \Infer{\semiflaming{Is $\ahat$ unsolved in $\Theta$?}}
              {\elimprop{\Gamma[\ahat]}{P}{\Theta} \\
               \instjudgl{\Theta}{\ahat}{B}{\Delta}
              }
              {\instjudgl{\Gamma[\ahat]}
                        {\ahat}
                        {P \implies B}
                        {\Delta}}
        \and
        \Infer{}
              {\checkprop{\Gamma[\ahat]}{P} \\
               \instjudgl{\Gamma[\ahat]}{\ahat}{B}{\Delta}
              }
              {\instjudgl{\Gamma[\ahat]}
                        {\ahat}
                        {B \with P}
                        {\Delta}}
      \end{mathpar}    
    %
    \\[-1.5ex]
    %
      \judgbox{\instjudgr{\Gamma}{\ahat}{A}{\Delta}}
         {Under input context $\Gamma$,
           instantiate $\ahat$ such that $A \subtype \ahat$,
           with output context $\Delta$}
      \begin{mathpar}
        \Infer{\InstRSolve}
                { \Gamma \entails \tau}
                { \instjudgr{\Gamma, \ahat, \Gamma'}
                            {\ahat}
                            {\tau}
                            {\Gamma, \hypeq{\ahat}{\tau}, \Gamma'}
                 }
        \and
        \Infer{\InstRReach}
                { }
                {\instjudgr{\Gamma[\ahat][\bhat]}
                           {\ahat}
                           {\bhat}
                           {\Gamma[\ahat][\hypeq{\bhat}{\ahat}]}}
        \and
        \Infer{\InstRArr}
              {\instjudgl{\Gamma[\ahat_2, \ahat_1, \hypeq{\ahat}{\ahat_1 \arr \ahat_2}]}
                        {\ahat_1}
                        {A_1}
                        {\Theta} \\
                 \instjudgr{\Theta}
                           {\ahat_2}
                           {[\Theta]A_2}
                           {\Delta}}
              {\instjudgr{\Gamma[\ahat]}
                         {\ahat}
                         {A_1 \arr A_2}
                         {\Delta}}
        \and 
        \Infer{\InstRAllL}
              {\instjudgr{\Gamma[\ahat], \MonnierComma{\bhat}, \bhat:\sort}{\ahat}{[\bhat/\beta]B}{\Delta, \MonnierComma{\bhat}, \Delta'}}
              {\instjudgr{\Gamma[\ahat]}{\ahat}{\alltype{\beta:\sort}{B}}{\Delta}}
        \\
        \Infer{}
              {\checkprop{\Gamma[\ahat]}{P} \\
               \instjudgr{\Gamma[\ahat]}{\ahat}{B}{\Delta}
              }
              {\instjudgr{\Gamma[\ahat]}
                        {\ahat}
                        {P \implies B}
                        {\Delta}}
        \and
        \Infer{\semiflaming{Is $\ahat$ unsolved in $\Theta$?}}
              {\elimprop{\Gamma[\ahat]}{P}{\Theta} \\
               \instjudgr{\Theta}{\ahat}{B}{\Delta}
              }
              {\instjudgr{\Gamma[\ahat]}
                        {\ahat}
                        {B \with P}
                        {\Delta}}
      \end{mathpar}

\caption{Instantiation}
\FLabel{fig:instantiation}
\end{figure*}

%
%
%


==> fig-decl-checkprop.tex <==
\begin{myfigure}[htbp]
  
  \loudjudgbox{declcheckprop}{\declcheckprop{\Psi}{P}}
          {Under context $\Psi$, check $P$}
  \begin{mathpar}
    \Infer{\DeclCheckpropEq}
         { }
         {\declcheckprop{\Psi}{(t = t)}}
  \end{mathpar}

  \caption{Declarative truth}
  \FLabel{fig:decl-checkprop}
\end{myfigure}

%
%
%


==> fig-hereditary.tex <==
\begin{figure}
\begin{mathpar}
\begin{array}{lcl}
\hsubst{\chk}{A}{e}{x}{x} & = & e \\ 
\hsubst{\syn}{A}{e}{x}{x} & = & (e:A) \\ 
\hsubst{\syn}{A}{e}{x}{e_1\;e_2} & = & \hsubst{\syn}
\end{mathpar}
\caption{Hereditary Substitution}
\label{fig:hereditary-substitution}
\end{figure}


%
%
%


==> fig-old-alg-subtyping.tex <==
\begin{figure*}[htbp]
  \judgbox{\subjudg{\Gamma}{A}{B}{\Delta}}%
     {Under input context $\Gamma$,
       type $A$ is a subtype of $B$, with output context $\Delta$}
  \begin{mathpar}
  \Infer{\SubVar}
              {\alpha \in \Gamma}
              {\subjudg{\Gamma}{\alpha}{\alpha}{\Gamma}}
  \and
  \Infer{\SubUnit}
            { }
            {\subjudg{\Gamma}{\unitty}{\unitty}{\Gamma}}
  \and
  \Infer{\SubExvar}
            { }
            {\subjudg{\Gamma[\ahat]}{\ahat}{\ahat}{\Gamma[\ahat]}}
  \and
  \Infer{\SubArr}
            {\subjudg{\Gamma}{B_1}{A_1}{\Theta} \\
              \subjudg{\Theta}{[\Theta]A_2}{[\Theta]B_2}{\Delta}}
            {\subjudg{\Gamma}{A_1 \arr A_2}{B_1 \arr B_2}{\Delta}}
  \\
  \Infer{\SubAllL}
            {\subjudg{\Gamma, \MonnierComma{\ahat}, \ahat:\sort}
                     {[\ahat/\alpha]A}
                     {B}
                     {\Delta, \MonnierComma{\ahat}, \Theta}}
            {\subjudg{\Gamma}{\alltype{\alpha:\sort}{A}}{B}{\Delta}}
  \and
  \Infer{\SubAllR}
            {\subjudg{\Gamma, \alpha:\sort}{A}{B}{\Delta, \alpha:\sort, \Theta}}
            {\subjudg{\Gamma}{A}{\alltype{\alpha:\sort}{B}}{\Delta}}
  \\
  \Infer{\SubInstL}
            {
              \ahat \notin \FV{%
                A}
              \\
              \instjudgl{\Gamma[\ahat]}{\ahat}{%
                   A}{\Delta}
            }
            {\subjudg{\Gamma[\ahat]}{\ahat}{A}{\Delta}}
  \and
  \Infer{\SubInstR}
            {
              \ahat \notin \FV{%
                A}
              \\
              \instjudgr{\Gamma[\ahat]}{\ahat}{%
                A}{\Delta}
            }
            {\subjudg{\Gamma[\ahat]}{A}{\ahat}{\Delta}}
  \\
  \Infer{\SubImpliesL}
        { \checkprop{\Gamma}{P} \\
          \subjudg{\Gamma}{A}{B}{\Delta} 
        }
        {
          \subjudg{\Gamma}{P \implies A}{B}{\Delta} 
        }
  \and
  \Infer{\SubImpliesR}
        { \addpropsubjudg{\Gamma}{P}{A}{B}{\Delta}
        }
        {\subjudg{\Gamma}{A}{P \implies B}{\Delta}}
  \\
  \Infer{\SubWithL}
        {
          \addpropsubjudg{\Gamma}{P}{A}{B}{\Delta}
        }
        {\subjudg{\Gamma}{P \with A}{B}{\Delta}}
  \and
  \Infer{\SubWithR}
        { \checkprop{\Gamma}{P} \\
          \subjudg{\Gamma}{A}{B}{\Delta} 
        }
        {
          \subjudg{\Gamma}{A}{B \with P}{\Delta} 
        }
  \\
  \Infer{\SubBot}
        { }
        {\subjudg{\bot}{A}{B}{\bot}}
  \end{mathpar}  

  \judgbox{\addpropsubjudg{\Gamma}{P}{A}{B}{\Delta}}%
     {Under input context $\Gamma$,
       \\
       check that $A$ is a subtype of $B$ under a context incorporating $P$,
       \\
       with output context $\Delta$}
  \begin{mathpar}
    \Infer{}
       {\elimprop{\Gamma}{P}{\bot}}
       {\addpropsubjudg{\Gamma}{P}{A}{B}{\Gamma}}
    \and
    \Infer{}
       {\elimprop{\Gamma, \MonnierComma{U}}{P}{\Thetac}
         \\
         \subjudg{\Thetac}{[\Thetac]A}{[\Thetac]B}{\Delta, \MonnierComma{U}, \Delta'}
       }
       {\addpropsubjudg{\Gamma}{P}{A}{B}{\Delta}}
  \end{mathpar}

  \caption{Algorithmic subtyping}
  \FLabel{fig:alg-subtyping}
\end{figure*}

\begin{figure}
  \judgbox{\checkprop{\Gamma}{P}}
          {Under context $\Gamma$, derive $P$}
  \begin{mathpar}
    \Infer{}
          { }
          {\checkprop{\bot}{P}}
    \and
    \Infer{}
          { [\Gamma]s = [\Gamma]t }
          {\checkprop{\Gamma}{s = t}}
  \end{mathpar}
  \judgbox{\elimprop{\Gamma}{P}{\Delta}}
          {Incorporate hypothesis $P$ into $\Gamma$, producing $\Delta$}
  \begin{mathpar}
    \Infer{}
          {}
          {\elimprop{\bot}{P}{\bot}}
    \and
    \Infer{}
          {\elimeq{\Gamma}{s}{t}{\Delta} }
          {\elimprop{\Gamma}{s = t}{\Delta}}
  \end{mathpar}


  \caption{Handling Propositions}
  \FLabel{fig:alg-prop}
\end{figure}


\begin{figure}
  \judgbox{\elimeq{\Gamma}{s}{t}{\Delta}}
          {Unify $s$ and $t$, taking $\Gamma$ to $\Delta$}
  \begin{mathpar}
    \Infer{}
          { }
          {\elimeq{\Gamma}{\zero}{\zero}{\Gamma}}
    \and
    \Infer{}
          {\elimeq{\Gamma}{s}{t}{\Delta}}
          {\elimeq{\Gamma}{\succ{s}}{\succ{t}}{\Delta}}
   \and
   \Infer{}
         {\insteq{\Gamma}{v}{t}{\Delta}}
         {\elimeq{\Gamma}{v}{t}{\Delta}}
  \and    
  \Infer{}
        {\insteq{\Gamma}{v}{t}{\Delta}}
        {\elimeq{\Gamma}{t}{v}{\Delta}}
  \\
  \Infer{}
        { }
        {\elimeq{\Gamma}{\zero}{\succ{t}}{\bot}}
  \and
  \Infer{}
        { }
        {\elimeq{\Gamma}{\succ{t}}{\zero}{\bot}}
  \end{mathpar}
  \judgbox{\insteq{\Gamma}{v}{t}{\Delta}}
          {Update $\Gamma$ to $\Delta$, in order to equate $v$ and $t$}
  \begin{mathpar}
  \Infer{}
        { }
        {\insteq{\Gamma[u:\ind][v:\ind]}{v}{u}{\Gamma[u:\ind][\hypeq{v:\ind}{u}]}}
  \and
  \Infer{}
        { }
        {\insteq{\Gamma[v:\ind][u:\ind]}{v}{u}{\Gamma[v:\ind][\hypeq{u:\ind}{v}]}}
  \and
  \Infer{}
        { }
        {\insteq{\Gamma[v:\ind]}{v}{\zero}{\Gamma[\hypeq{v:\ind}{\zero}]}}
  \and
  \Infer{}
        {\insteq{\Gamma[u:\ind,\hypeq{v:\ind}{\succ{u}}]}
                {u}{t}
                {\Delta}
        }
        {\insteq{\Gamma[v:\ind]}{v}{\succ{t}}{\Delta}}
  \end{mathpar}
  \caption{Solving Equations}
  \label{fig:alg-elimeq}
\end{figure}
%
%
%


==> fig-pattern-subst.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


\begin{figure}[htbp]
\loudjudgbox{untypedpatsjudg}{\untypedpatsjudg{\vvec}{\Pi}{e'}}{untypedpatsjudg}
%
  \begin{mathpar}
    \Infer{}
        {}
        {\untypedpatjudg{\cdot}{\cdot}{e}{e}}
    \and
    \Infer{}
        {\untypedpatjudg{v_0, \vvec}{p_0, \pvec}{e}{e'}}
        {\arrayenvbl{\untypedpatjudg{\inl{v_0}, \vvec}{\pvec}{e}{e'}
         \\
         \untypedpatjudg{\inr{v_0}, \vvec}{\pvec}{e}{e'}}}
    \\
    \Infer{}
        {\untypedpatjudg{v_1, v_2, \vvec}{p_1, p_2, \pvec}{e}{e'}}
        {\untypedpatjudg{\pair{v_1}{v_2}, \vvec}{\pair{p_1}{p_2}, \pvec}{e}{e'}}
    \and
    \Infer{}
        {\untypedpatjudg{\vvec}{p_1, p_2, \pvec}{e}{e'}}
        {\untypedpatjudg{\unitexp, \vvec}{\unitpat, \pvec}{e}{e'}}
    \\
    \Infer{}
        {\untypedpatjudg{\vvec}{\pvec}{[v_0 / x]e}{e'}}
        {\untypedpatjudg{v_0, \vvec}{x, \pvec}{e}{e'}}
    \and
    \Infer{}
        {\untypedpatjudg{\vvec}{\pvec}{e}{e'}}
        {\untypedpatjudg{v_0, \vvec}{\wild, \pvec}{e}{e'}}
    \\
    \Infer{}
        {\untypedpatsjudg{\vvec}{\Pi_1}{e'}}
        {\untypedpatsjudg{\vvec}{\Pi_1 \alt \Pi_2}{e'}}
    \and
    \Infer{}
        {\notuntypedpatsjudg{\vvec}{\Pi_1}
         \\
         \untypedpatsjudg{\vvec}{\Pi_2}{e'}
        }
        {\untypedpatsjudg{\vvec}{\Pi_1 \alt \Pi_2}{e'}}
  \end{mathpar}
  \caption{Untyped pattern substitution}
  \FLabel{fig:untyped-pattern-subst}
\end{figure}

%
%
%


==> fig-type-assignment.tex <==

\begin{figure}[t]
\loudjudgbox{judge}{\judge{\Psi}{e}{A}}{Under context $\Psi$, $e$ has type $A$}
\begin{mathpar}
\Infer{\AssignVar}
      {x:A \in \Psi}
      {\judge{\Psi}{x}{A}}
\and
\Infer{\AssignUnit}
      { }
      {\judge{\Psi}{\unitexp}{\unitty}}
\\
\Infer{\AssignArrIntro}
      {\judge{\Psi, x:A}{e}{B}}
      {\judge{\Psi}{\lam{x} e}{A \arr B}}
\and
\Infer{\AssignArrElim}
      {\judge{\Psi}{e_1}{A \arr B} \\
       \judge{\Psi}{e_2}{A}}
      {\judge{\Psi}{e_1\;e_2}{B}}
\\
\Infer{\AssignAllIntro}
      {\judge{\Psi, \alpha}{e}{A}}
      {\judge{\Psi}{e}{\alltype{\alpha}{A}}}
\and
\Infer{\AssignAllElim}
      {\judge{\Psi}{e}{\alltype{\alpha}{A}} \\
       \judgetp{\Psi}{\tau}}
      {\judge{\Psi}{e}{[\tau/\alpha]A}}    
\end{mathpar}
\caption{Type assignment rules for predicative System F}
\FLabel{fig:type-assignment}
\end{figure}



%
%
%


==> fig-unification.tex <==
\begin{figure}
\judgbox{\unify{\Psi}{t_1}{t_2}{\theta}}
    {Under $\Psi$, substitution $\theta$ unifies $t_1$ and $t_2$}

\begin{mathpar}
\Infer{\UnifyVarL}
      { u \notin \FV{t} }
      { \unify{\Psi}{u}{t}{t/u} }

\and

\Infer{\UnifyVarR}
      { u \notin \FV{t}
        \\
        t \mbox{ not a variable}
      }
      { \unify{\Psi}{t}{u}{t/u} }

\and

\Infer{\UnifyCon}
      { \unify{\Psi}{\vec{t_1}}{\vec{t_2}}{\theta} }
      { \unify{\Psi}{f(\vec{t_1})}{f(\vec{t_2})}{\theta} }

\\

\Infer{\UnifySeqNil}
      { }
      { \unify{\Psi}{\cdot}{\cdot}{\idsubst} }

\and 
    
\Infer{\UnifySeqCons}
      { \unify{\Psi}{t_1}{t_2}{\theta}
        \\
        \unify{\Psi}{\theta(\vec{t_1})}{\theta_0(\vec{t_2})}{\theta'}
      }
      { \unify{\Psi}{(t_1, \vec{t_1})}{(t_2, \vec{t_2})}{\theta' \circ \theta} }
\end{mathpar}


\caption{Martelli-Montanari unification}
\FLabel{fig:unification}
\end{figure}


%
%
%


==> flags-draft.tex <==
\def\OPTIONLoudLabels{0}


==> flags-final.tex <==
\def\OPTIONLoudLabels{0}


==> grue.tex <==
\begin{figure*}
\newcommand{\Room}[2]{
  \begin{tabular}[t]{l}
    \textcolor{dBlue}{\textvtt{\Backslash{#1}}}
    \\{}
    \ensuremath{#2}
  \end{tabular}
}

    \begin{tikzpicture}
      [auto, node distance=2cm, >=latex,  %
       descr/.style= {fill=white, inner sep=5pt, anchor=center}
      ]
      \node (inst) {\Room{instjudg}{\instjudg{\Gamma}{\ahat}{t}{\sort}{\Delta}}};
      \node [below of=inst, left=60pt, node distance=40pt] (checkeq) {\Room{checkeq}{\checkeq{\Gamma}{t_1}{t_2}{\sort}{\Delta}}};
      \draw [->] (checkeq) -- (inst);
 %
%
%
      \node [below of=checkeq, left=50pt, node distance=60pt] (checkprop) {\Room{checkprop}{\checkprop{\Gamma}{P}{\Delta}}};
      \draw [->] (checkprop) -- (checkeq);
%
%
      \node [below of=checkeq, node distance=50pt] (propequiv) {\Room{propequivjudg}{\propequivjudg{\Gamma}{P}{Q}{\Delta}}};
      \draw [->] (propequiv) -- (checkeq);
      \node [below of=propequiv, right=10pt, node distance=40pt] (equiv) {\Room{equivjudg}{\equivjudg{\Gamma}{A}{B}{\Delta}}};
      \node [below of=equiv, node distance=50pt] (sub) {\Room{subjudg}{\subjudg[\polvar]{\Gamma}{A}{B}{\Delta}}};
%
%
%
%
      \draw [->] (equiv) -- (propequiv);
      \draw [->] (equiv) -- (inst);
      \draw [->] (sub) -- (equiv);

      \node [below of=sub, node distance=60pt] (chk) {\Room{chkjudg}{\chkjudg{p}{\Gamma}{e}{A}{\Delta}}};
      \node [below of=chk, node distance=60pt] (syn) {\Room{synjudg}{\synjudg{p}{\Gamma}{e}{B}{\Delta}}};
      \draw [->] (chk) -- (sub);
%
      \node [left of=syn, node distance=140pt] (recspine) {\Room{recspinejudg}{\recspinejudg{\Gamma}{s}{A}{p}{B}{q}{\Delta}}};
      \node [above of=recspine, node distance=60pt] (spine) {\Room{spinejudg}{\spinejudg{\Gamma}{s}{A}{p}{B}{q}{\Delta}}};
      \draw [->] (spine) -- (checkprop);
      \draw [->] (syn) -- (recspine);
      \draw [->] (recspine) -- (spine);
      \draw [<->] (chk) -- (syn);
      \draw [->] (chk) -- (checkprop);
      \draw [->] (spine) -- (chk);
      \node [right of=syn, node distance=140pt] (match) {\Room{matchjudg}{\matchjudg{p}{\Gamma}{\Pi}{\Avec}{C}{\Delta}}};
      \node [right of=chk, node distance=160pt] (elimeq) {\Room{elimeq}{\elimeq{\Gamma}{s}{t}{\sort}{\Deltabot}}};
      \node [right of=sub, right=50pt, node distance=50pt] (covers) {\Room{covers}{\covers{\Gamma}{\Pi}{\Avec}}};
      \draw [<->] (match) -- (chk);
      \draw [->] (match) -- (elimeq);
      \draw [->] (covers) -- (elimeq);
      \draw [->] (chk) -- (covers);


%
%
    %

%
%
%
     %
    \end{tikzpicture}

\caption{A maze of twisty judgments, all alike}
\FLabel{fig:grue}
\end{figure*}


==> real-flags-draft.tex <==
\def\OPTIONLoudLabels{1}

